Verification of Neural Network Control Policy Under Persistent Adversarial Perturbation

Deep neural networks are known to be fragile to small adversarial perturbations. This issue becomes more critical when a neural network is interconnected with a physical system in a closed loop. In this paper, we show how to combine recent works on neural network certification tools (which are mainly used in static settings such as image classification) with robust control theory to certify a neural network policy in a control loop. Specifically, we give a sufficient condition and an algorithm to ensure that the closed loop state and control constraints are satisfied when the persistent adversarial perturbation is l-infinity norm bounded. Our method is based on finding a positively invariant set of the closed loop dynamical system, and thus we do not require the differentiability or the continuity of the neural network policy. Along with the verification result, we also develop an effective attack strategy for neural network control systems that outperforms exhaustive Monte-Carlo search significantly. We show that our certification algorithm works well on learned models and achieves 5 times better result than the traditional Lipschitz-based method to certify the robustness of a neural network policy on a cart pole control problem.

==> 5_Experiments_old.tex <==
%\todo[inline]{What examples are we going to show here?}
%We need a killer example here...
%MuJoCo

% Simple classical control: Inverted pendulum, double inverted pendulum, quadruple inverted pendulum
% \begin{enumerate}
%     \item Code the physics-based simulator: discretize the continuous time nonlinear equation
%     \item Assume that the physics parameters are partially known -- model the uncertainty set
%     \item Linearize the dynamic with nonlinear equation
%     \item Train a neural network policy for stabilization -- consider using both deep deterministic policy gradient (DDPG) and DQN (discontinuous control strategy)
%     \item Neural network robustness certification
%     \item Find closed loop invariant set, prove robust stability (check how to calculate the $\mathcal{H}_\infty$ and the $\mathcal{L}_1$ norms).
%     \item Demonstrate adversarial attack 
% \end{enumerate}

%In this section, we test our algorithm on a cart-pole control problem. We first certify the state constraint requirement on the linearized dynamic with persistent adversarial perturbation and compare the tightness of Algorithm \ref{alg:lin} versus the traditional Lipschitz based method (Theorem \ref{lemma:L1}) from robust control theory. Then, we demonstrate an example to certify the state constraint requirement with nonlinear dynamics, uncertainty on model parameters, and quantized control action.
We test our algorithm on a cart-pole control problem. We first certify the state constraint requirement on the linearized dynamic with persistent adversarial perturbation and analyze the tightness of Algorithm \ref{alg:lin}. Note that we cannot directly compare our method with the existing literature~\cite{berkenkamp2017safe, jin2018stability, jin2018control, richards2018lyapunov} because these methods cannot handle persistent adversarial perturbation with bounded $\ell_\infty$ yet unbounded $\ell_2$ norm. Instead, we use the result from Lemma \ref{lemma:L1} as our baseline because it is derived from robust control theory with similar assumption on Lipschitz continuity. We show that Algorithm \ref{alg:lin} can certify the state constraint requirement with larger adversarial perturbation compared to the Lipschitz-based method (Lemma \ref{lemma:L1}. 
%versus the traditional Lipschitz based method (Theorem \ref{lemma:L1}) from robust control theory. 
Finally, we show an example to certify the state constraint requirement with nonlinear dynamics, model uncertainty, and quantized control action.
%Lipschitz based method (Theorem \ref{lemma:L1}) from robust control theory


%Test different NN certification algorithm (from exact solution to approximated solution)
%Compare the tightness of the invariant set based method vs Lipschitz based method.
%Expected result: the invariant set based method is tighter because we tend to over-estimate the Lipschitz constant.

%\textcolor{blue}{May need to compare with other people's method}

%More advanced example (with image classifier in between): how do we derive the plant model in this case?

% \subsection{System model}
% We consider a cart-pole problem with $\eta$ being the displacement of the cart and $\theta$ the angle of the pole. The dynamics is given by
% \begin{subequations}
% \begin{align}
% \Ddot{\eta} &= \Big(\frac{4}{3}(M+m)l - ml \text{cos}^2(\theta)\Big)^{-1} (\frac{4}{3}ml^2 \dot{\theta}^2 \text{sin}(\theta) - mgl\text{sin}(\theta)\text{cos}(\theta) + \frac{4}{3}lu )\nonumber\\
% \Ddot{\theta} &= \Big(\frac{4}{3}(M+m)l - ml \text{cos}^2(\theta)\Big)^{-1}(-ml\dot{\theta}^2\text{sin}(\theta)\text{cos}(\theta) + (M+m)g\text{sin}(\theta) - \text{cos}(\theta)u) \nonumber
% \end{align}\label{eq:nonlinear_cont}
% \end{subequations}
% Using Euler discretization, the nonlinear discrete time cart pole model is given by
% \begin{equation}
%     \eta[t+1] = \eta[t] + \tau \dot{\eta}[t], \, \dot{\eta}[t+1] = \dot{\eta}[t] + \tau \Ddot{\eta}[t], \, \theta[t+1] = \theta[t] + \tau \dot{\theta}[t], \, \dot{\theta}[t+1] = \dot{\theta}[t] + \tau \Ddot{\theta}[t] \nonumber
% \end{equation}
% with sampling time $\tau$. Define the state vector $x = \begin{bmatrix} \eta & \dot{\eta} & \theta & \dot{\theta}\end{bmatrix}^\top$. The linearized model around the origin is given by $x[t+1] = A x[t] + B u[t]$ with
% \begin{equation}
% A = \begin{bmatrix}1 & \tau & 0 & 0 \\ 0 & 1 & \frac{-3mg\tau}{4M+m} & 0 \\ 0 & 0 & 1 & \tau \\ 0 & 0 & \frac{3(M+m)g\tau}{(4M+m)l} & 1\end{bmatrix}, \quad B = \begin{bmatrix} 0 \\ \frac{4\tau}{4M+m} \\ 0 \\ \frac{-3\tau}{(4M+m)l}\end{bmatrix}. \label{eq:linear_disc}
% \end{equation}

\subsection{Experiment setup}
We use the cart-pole environment from stable baselines~\cite{stable-baselines} with default model parameters. We use proximal policy optimization (PPO)~\cite{schulman2017proximal} to train a $3$-layer neural network policy with continuous control output. Each layer has $16$ neurons, and the activation function is ReLU.
%stable baselines \cite{stable-baselines} with 1M iteration. We update the environment to allow continuous control action, and set the state constraint to be $6$ degrees. 
We note that many trained neural network policies can obtain perfect reward in the training environment, but will eventually violate the state constraints if we simulate the closed loop dynamics for a longer horizon. To obtain a more stable neural network policy, we modify the reward function to be
%However, if we simulate the closed loop dynamics for a longer horizon, the state constraint could eventually be violated. To avoid this issue, we modify the reward function to be
%many neural networks trained by reinforcement learning algorithms can obtain perfect rewards in certain task, but the policies are indeed locally \emph{unstable} according to the conditions from Lemma \ref{lemma:local}. This is because we do not explicitly incorporate the stability as a requirement into the reward function.
\begin{equation}
    r[t] = 2 - \frac{x[t]^\top Q x[t] + u[t]^\top R u[t]}{x_{lim}^\top Q x_{lim} + u_{lim}^\top R u_{lim}}, \nonumber
\end{equation}
which will attempt to minimize the LQR cost $x[t]^\top Q x[t] + u[t]^\top R u[t]$. 
%This helps to stabilize the closed loop dynamic for certification analysis. 
The policy is trained with $2$M steps. The objective is to certify that the angle of the pole will stay within $5$ degrees. We use the method proposed in~\cite{weng2018towards} as the neural network certification tool.

\subsection{Certification with linearized dynamics}
% -- Compare the tightness of Theorem 1 vs Theorem 2 by finding the max allowable perturbation on each sensor and actuator (5 by 2 table)
% -- What are the certified bounds for each case? Compare with the max observed state deviation and calculate the ratio
% -- Attack the system: what is the minimum distortion to break the system? 
% -- May want to discuss the tightness of different NN certification tool
In this subsection, we linearize the cart-pole model around the closed loop equilibrium, and certify the state constraint requirement on the linearized model. %As an illustrative example, we consider the adversarial perturbation on the measurement of the angle of the pole, which is an important input to the neural network policy. Before the certification work, 
We first demonstrate the effectiveness of our attack algorithm described in Section \ref{sec:attack_algo} in Figure \ref{fig:response}.
%We find out it is possible to force state constraint violation by injecting a sensor perturbation with magnitude only equal to XXX degrees using our attack algorithm described in Section \ref{sec:attack_algo}. Figure XXX shows that our attack algorithm is extremely effective. 
If we use random perturbation to attack the system, even if we run the simulation with $10^5$ time steps, the maximum observed state deviation is only $0.59$ degrees, with standard deviation being $0.17$ degrees. %One may falsely conclude that it is safe to stay within six times the standard deviation by assuming that the state deviation follows a Gaussian distribution. 
In Figure \ref{fig:response}, we inject our designed attack between time $100$s and $180$s with the same attack level ($0.88$ degrees error on angle measurement), and the maximum state deviation is above $5$ degrees, which is $29$ standard deviation away.
%times of the standard deviation. Indeed, when we increase the attack level to $0.67$ degrees, the system becomes unstable and the state deviation goes to infinity. 
This shows that our deliberate design of attack sequence is extremely effective. 

\begin{figure}[t!]
      \centering
      \includegraphics[width=0.9\textwidth]{AttackResponse.pdf}
      \caption{The left figure is the attack signal on the angle measurement and the right figure is the angle of the pole. Our designed attack is injected between $100$s and $180$s.}
      \label{fig:response}
\end{figure}

%Before the certification task, we first implement our attack algorithm in Section \ref{sec:attack_algo}
%to find an upper bound of the 
We implement $5$ different attacks on the control action and the $4$ state measurements and the result is summarized in Table \ref{tab:attack-L1}. In Table \ref{tab:attack-L1}, the attack column is the attack level that cause state constraint violation found by our attack algorithm. The next column is the certified robustness calculated by Algorithm \ref{alg:lin}. The Lipschitz-based column is the robustness calculated based on traditional robust control theory (Lemma \ref{lemma:L1} with $\gamma_\pi$ sampled in a local region), which serves as the baseline for comparison. We estimate the local Lipschitz constant based on Monte-Carlo simulation, so it is only a lower limit and does not offer a certificate. Even when the comparison is in favor of the Lipschitz-based approach, our method can certify an attack level that is in average $5$ times larger than the one from the Lipschitz-based approach. This shows the significance of our method.

\input{_tab_result.tex}
%To the certification test, we first run Algorithm \ref{alg:lin} to certify that the state constraint is satisfied for perturbation with magnitude up to $0.08$ degrees. We then calculate an upper bound of the local Lipschitz constant of the neural network policy, and use Theorem \ref{lemma:L1} to conclude that the system is locally input-output stable when the perturbation magnitude is less than $0.05$ degrees. Note that Algorithm \ref{alg:lin} allows us to certify a perturbation with larger magnitude. We calculate the tightness of our two methods on each type of attack and summarize the result in Table 1.

Nevertheless, there is still a gap between our certified robustness and the minimal attack level. The gap is contributed by at least three factors.
%There are several factors that contribute to the gap between our certification bound and the minimal perturbation found. 
First, the neural network certification tool calculates an over-approximation set of the neural network output layer by layer, which is conservative.
%The gap for the best polynomial time algorithm for a $3$ layers neural network has a factor about $3$. S
Second, Theorem \ref{thm:LTI} is only a sufficient condition. Indeed, the residual control policy $\bar{u_0}$ in Algorithm \ref{alg:lin} is treated as adversarial as well, which is conservative. Third, although our attack algorithm is very effective, it is sub-optimal.
%To quantify the conservatism of each component, we use Monte Carlo simulations to replace the neural network certification tool, and the gap is reduced to XXX. 
%To estimate the contribution of each factor, we use Monte-Carlo simulation to replace the neural network certification tool and the gap drop from $13.7$ to $6$. Therefore,
Our estimate is that the neural network certification tool contributes to a factor of $2$ to $3$ of the gap, and Theorem \ref{thm:LTI} and our attack algorithm contributes to a factor of $4$ to $5$ of the gap. We note that the gap also highly depends on the nonlinearity of the neural network model. The additional experiments are included in the supplementary material. One neural network is trained by behavior cloning of a LQR policy. This network is more linear and thus the gap between the minimal attack and the certified robustness is only $2.4$. Another network is a $3$-layer network with $32$ neurons at each layer. This network is more nonlinear and thus the gap is larger. However, our method becomes $16$ times better than the Lipschitz-based method in this network.

%Our estimate is that the neural network certification tool contributes to a factor of $2$ to $3$ in the gap, while Theorem \ref{thm:LTI} contributes to a factor of $3$ to $4$. 
%We compare the tightness of the invariant set based method and the Lipschitz based method. We observe the invariant set based method in Theorem \ref{thm:LTI} can certify a large range of adversarial attack. Specifically, we can guarantee that the state and input constraints are satisfied when the measurement of the pole angle has a perturbation up to $1.5$ degrees.

\subsection{Certification with nonlinear dynamics, uncertain parameters, and quantized action} \label{sec:exp_nonlinear}
%The previous experiment assumes that the system dynamic is linear and the model parameters are perfectly known. 
In this experiment, the neural network is interconnected with the original nonlinear model, with some uncertainty on the model parameters. We also assume the neural network output is quantized -- this makes the neural network policy discontinuous and non-differentiable (the Lipschitz constant becomes infinity). Indeed, the closed loop system does not have a stable equilibrium. Even in this case, we can still apply Theorem \ref{thm:LTI} to certify that the requirement \eqref{eq:goal} is satisfied under persistent adversarial attack \eqref{eq:attack}.
%The purpose of this experiment is to show the capability of Theorem \ref{thm:LTI}.
%Note that quantized control action (control action is chosen in a discrete set) is very common in reinforcement learning problems. 
% With some math, we can show that the linearization error is upper bounded by
% \begin{subequations}
% \begin{align}
% | \delta_\eta | &\leq \tau \Big[ |\frac{12m\text{sin}^2(\bar{\theta})}{(4M+m)^2}| |u| + |\frac{6mg\bar{\theta}}{(4M+m)\pi} + \frac{9m^2 g\text{sin}^2(\bar{\theta})}{(4M+m)^2}| |\theta| + |\frac{4ml\text{sin}(\bar{\theta})\bar{\dot{\theta}}}{4M+m}| |\dot{\theta}| \Big] \nonumber\\
% | \delta_\theta | &\leq \tau \Big[ |\frac{3(1-\text{cos}(\bar{\theta}))}{(4M+m)l} + \frac{3m\text{sin}^2(\bar{\theta})}{(4M+m)^2 l}| |u| + |\frac{3(M+m)g\bar{\theta}}{(4M+m)l\pi} + \frac{9m(M+m)g\text{sin}^2(\bar{\theta})}{(4M+m)^2 l}| |\theta| \nonumber\\
% & + |\frac{1.5m\text{sin}(2\bar{\theta})\bar{\dot{\theta}}}{4M+m}| |\dot{\theta}| \Big] \nonumber
% \end{align}\label{eq:err_bnd}
% \end{subequations}
%where $\delta_\eta$ is the uncertainty-induced perturbation on the second state, $\delta_\theta$ is the perturbation on the fourth state, and $(\bar{\theta}, \bar{\dot{\theta}})$ are the maximum $\theta$ and $\dot{\theta}$ that have been observed. This allows us to bound the induced norm from $\alpha = [x; u]$ to $\delta$. For the uncertainty in model parameter, we assume that the length of the pole $l$ can vary within $\pm 5\%$. This uncertainty can also be absorbed into the block $\ttf{\Delta}$ in Figure \ref{fig:model}. The control action is quantized into a level of $0.1$ -- this part is added to the $\bar{u_0}$ in Line $11$ of Algorithm \ref{alg:lin}.
We bound the linearization error into the uncertainty block $\ttf{\Delta}$. Unlike the assumption we made in Algorithm \ref{alg:lin}, the norm of $\ttf{\Delta}$ is a function of the linearized region $\bar{x}$, and thus $\gamma_\Delta$ needs to be updated at each iteration. For the uncertainty in model parameter, we assume that the mass of the pole can vary within $\pm 10\%$. The control action is quantized into a level of $0.1$ -- this part is added to $\bar{u_0}$ in Algorithm \ref{alg:lin}. With all additional constraints, our certification level drops from $0.075$ degrees to $0.013$ degrees for the attack on pole angle measurement. 
%, while the minimal perturbation to totally break the system is reduced from $0.67$ degrees to $0.65$ degrees. 
When there are model uncertainty and quantization, our method becomes more conservative because we are dealing with the worst-case scenario where the model mismatch and the quantization error are treated as adversarial. Future research direction is to find a better characterization of the uncertainty set, which can make our method less conservative. 
%We repeat the same experiment and summarize the result in Table XXX.
%The adversarial perturbation in this experiment is on the sensor measurement for the angle of the pole. We certify the state constraint with adversarial perturbation up to $0.15$ degree. 

%Our strategy is to bound the linearization error over a region into the
%-- Bound the linearization error into the uncertainty set
%-- Characterize the model uncertainty due to parameters
%-- Quantized control action: not Lipschitz continuous, no stable equilibrium, no Lyapunov function -- Theorem 1 still apply
%-- Repeat the same experiments
%\subsection{Experiment 2: certification with known nonlinear dynamics}
%\subsection{Experiment 3: certification with nonlinear dynamics with uncertain model parameters}


==> _App_additional_result.tex <==
\section*{Appendix C: additional experiment result and discussion}

\textcolor{red}{TODO: need to rewrite this section as well.}

Here we provide some additional experiment results. The first neural network demonstrated in this section has an identical architecture to the one shown in Section \ref{sec:experiment} -- it is a $3$-layer neural network with $16$ neurons in each layer. The only difference is that this neural network is trained by behavior cloning of a LQR policy. The trained neural network policy is more linear around the equilibrium. Thus our certification method, which is based on linear robust control theory, is tighter. Table \ref{tab:add} shows our simulation result on this network model. If we compare Table \ref{tab:add} with Table \ref{tab:attack-L1}, we can see that the gap between the attack and the certified robustness decrease significantly. However, we also notice that the gap between our method (Algorithm \ref{alg:lin}) and the Lipschitz-based method becomes negligible. Therefore, our method offers less additional value on this network. For the network demonstrated in Section \ref{sec:experiment}, the neural network is highly nonlinear near the equilibrium point. In that case, Algorithm \ref{alg:lin} gives a significant advantage over the traditional Lipschitz-based method. 

\begin{table}[h!]
\centering
\caption{Additional comparison between the minimal attack distance and the certified robustness. This neural network is trained by behavior cloning of a LQR policy.}
\begin{adjustbox}{max width=1\textwidth}
    \begin{tabular}{c|c|c|c|cccc}
    \hline
    attack node & attack & Algo \ref{alg:lin} (Thm \ref{thm:LTI}) & Lipschitz-based & $\bar{x_1}$ & $\bar{x_2}$ & $\bar{x_3}$ & $\bar{x_4}$ \\
    \hline
      $u$ & 0.74219	& 0.34873	& 0.34873	& 0.39997	& 0.34454	& 2.32893	& 6.87542 \\
    $x_1$ & 0.83984	& 0.26523	& 0.26523	& 0.27679	& 0.23844	& 1.61170	& 4.75796\\
    $x_2$ & 0.34180	& 0.14482	& 0.14482	& 0.35430	& 0.30521	& 2.06306	& 6.09054\\
    $x_3$ & 1.39648	& 0.63789	& 0.63789	& 0.39066	& 0.33653	& 2.27474	& 6.71543 \\
    $x_4$ & 5.46875	& 2.38867	& 2.38867	& 0.37491	& 0.32296	& 2.18302	& 6.44465 \\
    \hline
    \end{tabular}%
    \end{adjustbox}
  \label{tab:add}%
\end{table}%

The second neural network is even more nonlinear than the one demonstrated in Section \ref{sec:experiment}. Table \ref{tab:add2} shows the result for a $3$-layer neural network with $32$ neurons at each layer. This network is more nonlinear near the equilibrium, and thus the gap between the minimal attack and the certified robustness become larger. Nevertheless, we also note that our certified robustness gives a significant advantage over the traditional Lipschitz-based method, with $16$ times improvement in average. 
%the neural network is highly nonlinear near the equilibrium point. In that case, Algorithm \ref{alg:lin} gives a significant advantage over the traditional Lipschitz-based method. 

\begin{table}[h!]
\centering
\caption{Additional comparison between the minimal attack distance and the certified robustness. This neural network has $3$ layers with $32$ neurons at each layer.}
\begin{adjustbox}{max width=1\textwidth}
    \begin{tabular}{c|c|c|c|cccc}
    \hline
    attack node & attack & Algo \ref{alg:lin} (Thm \ref{thm:LTI}) & Lipschitz-based & $\bar{x_1}$ & $\bar{x_2}$ & $\bar{x_3}$ & $\bar{x_4}$ \\
    \hline
      $u$ & 1.18164	& 0.02236	& 0.00166	& 0.01015 & 0.02522 & 0.24085 & 0.79849 \\
    $x_1$ & 0.21094	& 0.00186	& 0.00010	& 0.01012 & 0.02514 & 0.24011 & 0.79650\\
    $x_2$ & 0.13086	& 0.00205	& 0.00010	& 0.01027 & 0.02552 & 0.24368 & 0.80829\\
    $x_3$ & 1.33008	& 0.02227	& 0.00166	& 0.01012 & 0.02514 & 0.24009 & 0.79607 \\
    $x_4$ & 3.78516	& 0.05811	& 0.00439	& 0.01008 & 0.02504 & 0.23915 & 0.79299 \\
    \hline
    \end{tabular}%
    \end{adjustbox}
  \label{tab:add2}%
\end{table}%
 


==> _tab_result.tex <==
% Lily defines

% \begin{table}[t!]
% \centering
% \caption{Comparison between the minimal attack distance and the certified robustness. There are five different attack node -- one on control $u$ and four on each state. The attack column gives an upper bound of minimum adversarial attack level and certified robustness is a certified lower bound of it. The last four columns are the certified bound for state $x$.}
% \begin{adjustbox}{max width=1\textwidth}
%     \begin{tabular}{c|c|ccccc}
%     \hline
%     attack node & attack & certified robustness  & $\bar{x_1}$ & $\bar{x_2}$ & $\bar{x_3}$ & $\bar{x_4}$ \\
%     \hline
%       $u$ & 0.32031 & 0.04375 &	0.04575	& 0.05841	& 0.41626 &	0.73155 \\
%     $x_1$ & 0.14258 &	0.02266	& 0.04285	& 0.0547	& 0.38985	& 0.68514\\
%     $x_2$ & 0.08398 &	0.00859	& 0.04038	& 0.05155	& 0.36741	& 0.64569\\
%     $x_3$ & 0.64941 &	0.07969	& 0.04488	& 0.05729	& 0.40828	& 0.71753 \\
%     $x_4$ & 0.82813 &	0.10088	& 0.04441	& 0.0567	& 0.40405	& 0.71010 \\
%     \hline
%     \end{tabular}%
%     \end{adjustbox}
%   \label{tab:attack-L1}%
% \end{table}%

\begin{table}[t!]
\centering
\caption{Comparison between the minimal attack distance and the certified robustness. The attack column is the minimal attack found by our attack algorithm, the Algo \ref{alg:lin} column is the certified robustness from Algorithm \ref{alg:lin}, and the Lipschitz-base column is the baseline robustness from robust control theory (Theorem \ref{lemma:L1}). The last four columns are the certified bounds for the state.}
\begin{adjustbox}{max width=1\textwidth}
    \begin{tabular}{c|c|c|c|cccc}
    \hline
    attack node & attack & Algo \ref{alg:lin} ( Thm \ref{thm:LTI}) & Lipschitz-based & $\bar{x_1}$ & $\bar{x_2}$ & $\bar{x_3}$ & $\bar{x_4}$ \\
    \hline
      $u$ & 0.85742	& 0.07979	& 0.01563 & 0.06049	& 0.09994	& 0.79062	& 1.89337 \\
    $x_1$ & 0.12500	& 0.00830	& 0.00156 & 0.05736	& 0.09476	& 0.74965	& 1.79523\\
    $x_2$ & 0.14844	& 0.01104	& 0.00234 & 0.05838	& 0.09645	& 0.76303	& 1.82739\\
    $x_3$ & 0.87500	& 0.07500	& 0.01484 & 0.05871	& 0.09700	& 0.76730	& 1.83733 \\
    $x_4$ & 2.50391	& 0.21689	& 0.04219 & 0.05967	& 0.09858	& 0.77985	& 1.86754 \\
    \hline
    \end{tabular}%
    \end{adjustbox}
  \label{tab:attack-L1}%
\end{table}%







==> v1_1_Intro.tex <==

% 1st paragraph: adversarial examples in neural networks
Deep neural networks (DNN) have become state-of-the-arts in a variety of machine learning tasks due to their superior performance over traditional machine learning models and sometimes even human. Yet, recent studies demonstrate they are surprisingly fragile -- take image classification task for example,  small and imperceptible adversarial perturbations on the natural images can easily manipulate neural networks predictions~\cite{szegedy2013intriguing}. Unfortunately, adversarial examples have been found in many common deep learning tasks: from object detection \cite{xie2017adversarial}, image captioning \cite{chen2017show}, reading comprehension \cite{jia2017adversarial}, speech recognition \cite{cisse2017houdini} to malware detection \cite{wang2017adversary}. 

% 2nd paragraph: neural network based policy in the loop
The existence of adversarial examples is particularly dangerous for mission-critical machine learning tasks that heavily rely on DNNs, such as security cameras and self-driving cars. \textcolor{blue}{Mickey discuss self-driving car and reinforcement learning here.} \textcolor{purple}{Second paragraph: extend to neural network based policy in the loop. Reinforcement learning is one example. Discuss the self-driving car example -- nonlinear dynamics with some uncertainty, use neural network to process camera data and generate control action (deep NN), external disturbance, including measurement noise (sensor noise, hardware quantization, saturation, discretization, delay in data processing,...), require stability and safety constraint.}


% 3rd paragraph: robustness certificate of neural networks
In view of adversarial examples, much research effort has recently been devoted to developing verification methods to quantify robustness of neural networks. Current mainstreams can be categorized into two classes: \textit{complete verification} and \textit{incomplete verification}. A \textit{complete verifier}, such as Reluplex~\cite{katz2017reluplex}, can solve for minimum adversarial distortion, which is the smallest magnitude (in $\ell_p$ norm) perturbation required to fool DNN's top-1 prediction. However, solving for minimum adversarial distortions is computationally expensive -- it is proved to be NP-Complete~\cite{katz2017reluplex}. Fortunately, it is still possible to find a non-trivial lower bound of minimum adversarial distortion (also known as robustness certificate) in polynomial-time by over-approximating input perturbation sets. Such verifiers are known as \textit{incomplete verifiers} and have become popular due to its capability to deliver non-trivial robustness certificate efficiently~\cite{weng2018towards,Gehr2018AI2,dvijotham2018dual,Boopathy2019cnncert}. 

% 4th paragraph: goal of this paper
The goal of this paper is to derive robustness certificate for a closed-loop system with neural network policy in the loop. \textcolor{blue}{Mickey finishes here.} \textcolor{purple}{Fourth paragraph: goal of this paper -- derive robustness certificate for a closed loop system with neural network policy in the loop (state constraints, stability, verification). We assume that at least partial knowledge of the plant model is available (cannot be entirely model free).}



\subsection{Related Works}
\todo[inline]{Literature review and comparison}
Compare with safe reinforcement learning: safety during the exploration and deployment phase, read (\cite{garcia2015comprehensive}, \cite{chow2018lyapunov})

Compare with stability-certified reinforcement learning: see \cite{berkenkamp2017safe}, \cite{jin2018stability}, \cite{jin2018control}, \cite{richards2018lyapunov}

Lipchitz constant + IQC

Hardware quantization, digitalization introduce discontinuity -- the Lipchitz constant is infinite, and the common tools such as IQC or Lyapunov analysis does not work for these type of systems. 

%\todo[inline]{What if y and u are moving around, not linearize at a fixed point?}

Compare with tree based policy verification: \cite{bastani2018verifiable}

\subsection{Notations} \label{sec:notation}
In this paper, we use lower case letters such as $x$ to denote vectors and upper case letters such as $A$ to denote matrices. For a square matrix $A$, we use $\rho(A)$ to denote its spectral radius, which is the largest absolute value of the eigenvalues of $A$. We use boldface letters such as $\tf x$ and $\tf{\Phi}$ to denote signals and transfer matrices in the frequency domain, respectively. Consider a time series signal $\{x[t]\}_{t=0}^\infty$. The unilateral $z$-transform of the time series $\{x[t]\}_{t=0}^\infty$ is given by $\tf x (z) = \sum_{t=0}^\infty z^{-t} x[t]$. We use $\Phi[t]$ to denote the $t$-th spectral component of a transfer matrix $\tf{\Phi}$, i.e., $\tf{\Phi}(z) = \sum_{t=0}^\infty z^{-t} \Phi[t]$. We use $\tf x$ and $\tf{\Phi}$ as shorthand of $\tf x(z)$ and $\tf{\Phi}(z)$ when the context makes it clear.

The frequency domain notation is particularly useful when analyzing the property of a dynamical system. Let $\tf{\Phi}$ be the transfer matrix mapping from signal $\tf x$ to signal $\tf y$, i.e., $\tf y = \tf{\Phi} \tf x$ in the frequency domain. The corresponding time domain equation is given by the convolution formula $y[t] = \sum_{\tau=0}^\infty \Phi[\tau] x[t-\tau]$. We use $\| \tf x \|_{\ell_p}$ to denote the standard $\ell_p$ norm of the signal $\tf x$ and use $\| \tf{\Phi} \|_{\mathcal{H}_\infty}$ to denote the $\mathcal{H}_\infty$ norm of the system $\tf{\Phi}$. We define the absolute operator $\text{abs}(\cdot)$ of a stable transfer matrix $\tf{\Phi}$ by $\text{abs}(\tf{\Phi}) = \sum_{t=0}^\infty | \Phi[t] |$. Note that each element of the transfer matrix $\tf{\Phi}$ is absolutely summable if and only if the transfer matrix $\tf{\Phi}$ is real rational and stable (see Page 113 - 114 of \cite{oppenheim1996signals}).

%\begin{equation}
%\text{abs}(\tf M) = \sum_{k=0}^\infty | M[k] |. \label{eq:element}
%\end{equation}
%We assume that each element of the transfer matrix $M$ is absolutely summable. (in Page 113 - 114 of the Signals and Systems textbook, stability is equivalent to absolutely summable / integrable for both discrete and continuous time)

Finally, we use calligraphic letters such as $\SigSp{U}$ and $\SigSp{W}$ to denote spaces for signals and systems. For instance, $\SigSp{W} = \{\tf w | \|\tf w\|_{\ell_p} \leq \gamma \}$ is a valid space for the signal $\tf w$ and $\SigSp{G} = \{\tf{\Phi} | \|\tf{\Phi}\|_{\mathcal{H}_\infty} \leq \gamma \}$ is a valid space for the system $\tf{\Phi}$. 


==> v1_2_prelim.tex <==
We begin with a brief introduction of the neural network certification tools developed in a static setting. We then give the problem statement of this paper.
\subsection{Robustness Certificate of Neural Networks}
\textcolor{red}{Lily to finish:}

\textcolor{blue}{Brief introduction of set-based neural network robustness certification}

\textcolor{blue}{Given a neural network policy $u = \pi(y)$, we have tools to show that $u = \pi(y) \in \SigSp{U}$ for all $y \in \SigSp{Y}$ for some set $\SigSp{U}$ and $\SigSp{Y}$. Examples: ReLUplex, Zico's LP method, Lily's work, DeepPoly}

Lily's work: $K_L y + b_L \leq \pi(y) \leq K_U y + b_U$
Zico's LP: $K_L^{(k)} y + b_L^{(k)} \leq \pi(y) \leq K_U^{(k)} y + b_U^{(k)}$ with multiple $k$
ReLUplex: can have non-convex set

%Under the norm-ball bounded threat model, for NNs with ReLU activation functions, although the minimum adversarial distortion gives the best possible certified robustness, solving it is indeed computationally intractable due to its NP-completeness complexity \cite{katz2017reluplex}. Alternatively, solving a non-trivial lower bound of the minimum distortion as a provable robustness certificate is a more promising option but at the cost of obtaining a more conservative robustness certificate. Some analytical lower bounds depending solely on model weights can be derived \cite{szegedy2013intriguing,peck2017lower,hein2017formal,raghunathan2018certified} but they are in general too loose to be useful or limited to 1 or 2 hidden layers. The robustness of NNs can be efficiently certified on ReLU activation~\cite{kolter2017provable,weng2018towards} and general activation~\cite{zhang2018crown} but mostly on models with fully-connected layers. \cite{dvijotham2018dual} can also be applied to different activation functions but their bound quality might decrease a lot as a trade-off between computational efficiency due to its `any-time` property. This paper falls within this line of research with an aim of providing both a general and efficient certification framework for CNNs (see Table \ref{table_comparison} for detailed comparisons).

%Although verification-based approaches can provide robustness certification, finding the minimum distortion (i.e., the maximum certifiable robustness) of NNs with ReLU activations has been shown to be an NP-complete problem \cite{katz2017reluplex}. While minimum distortion can be attained in small and shallow networks  \cite{katz2017reluplex,lomuscio2017approach,cheng2017maximum,fischetti2017deep}, these approaches are not even scalable to moderate-sized NNs. Recent works aim to circumvent the scalability issue by efficiently solving a non-trivial lower bound on the minimum distortion \cite{kolter2017provable,weng2018towards,dvijotham2018dual}. However, existing methods may lack generality in supporting different network architectures and activation functions. In addition, current methods often deal with convolutional layers by simply converting back to fully-connected layers, which may lose efficiency if not fully optimized with respect to the NNs, as demonstrated in our experiments. To bridge this gap, we propose CNN-Cert, a general and efficient verification framework for certifying robustness of a broad range of convolutional neural networks (CNNs). The generality of CNN-Cert enables robustness certification of various architectures, including convolutional layers, max-pooling layers batch normalization layers and residual blocks, and general activation functions. The efficiency of CNN-Cert is optimized by exploiting the convolution operation. A full comparison of verification-based methods is given in Table \ref{table_comparison}.

\subsection{Problem Statement}
\begin{figure}[h!]
      \centering
      \includegraphics[width=0.8\textwidth]{NN_FB2.pdf}
      \caption{A neural network policy interconnected with a dynamical system.}
      \label{fig:model}
\end{figure}
In this paper, we consider a neural network policy interconnected with a dynamical system, as shown in Figure \ref{fig:model}. 
%We assume that the dynamics of the plant $\tf{P}$ is known. 
%The model architecture is shown in Figure \ref{fig:model}, where $\pi(\cdot)$ is a neural network control policy, $\tf{P}$ is a discrete time dynamical system with known dynamics, and $\ttf{\Delta}$ models the uncertainty of the system. 
Mathematically, Figure \ref{fig:model} is described by the following equations:
\begin{subequations}
\begin{align}
x[t+1] &= f(x[t], u[t], w[t], \delta[t]) \label{eq:g1}\\
y[t] &= g(x[t], w[t]) \label{eq:g2} \\
\alpha[t] &= h(x[t], u[t], w[t]) \label{eq:g3} \\
u[t] &= \pi(y[t]) \label{eq:g4} \\
\ttf{\delta} &= \Delta(\ttf{\alpha}) \label{eq:g5}.
\end{align}
\end{subequations}
%with the neural network policy $u[t] = \pi(y[t])$ and the uncertainty-induced input $\ttf{\delta} = \Delta(\ttf{\alpha})$. 
where $t$ denotes the time index, $x$ the state vector, $u$ the control action, and $y$ the measurement. The external perturbation $w$ of the system can be either adversarial or non-adversarial, and it can affect both the neural network input $y$ and the state $x$. We assume that $x = 0$ is an equilibrium of the system, i.e., $0 = f(0, 0, 0, 0)$.

\begin{remark}
Note that the neural network policy $u[t] = \pi(y[t])$ is assumed to be a static policy. If the neural network policy depends on a finite length of historical measurement, i.e., $u[t] = \pi(y[t], y[t-1],\dots,y[t-T])$ for a finite length $T$, then we can simply augment the state $x$ and measurement $y$ for $T$ steps and convert it to the form similar to \eqref{eq:g1} - \eqref{eq:g5}. The uncertainty block $\ttf{\Delta}$ can be dynamic, i.e., $\delta[t]$ is a function of $\alpha[k]$ for all $k \leq t$, and thus \eqref{eq:g5} is written in the frequency domain as opposed to the time domain formulation \eqref{eq:g1} - \eqref{eq:g4}.
\end{remark}
\begin{remark}
Note that $y$ in \eqref{eq:g2} is not a direct function of $u$ and $\delta$, and $\alpha$ in \eqref{eq:g3} is not a direct function of $\delta$. This assumption ensures that there is no algebraic loop in the equation, and the feedback structure in Figure \ref{fig:model} is well-posed. 
\end{remark}
\textcolor{blue}{May want to add a remark about the generality of this formulation}
%This form is very general: nonlinear dynamic, output feedback, un-modeled dynamic in both the state equation and the output equation, explicitly taking into account the external disturbance, very loose assumption on the neural network policy $\pi$ (can be discontinuous, non-differentiable)

%f, g known, $\Delta_f$, $\Delta_g$ unknown but satisfy certain constraints, $w$ is contained with some pre-specified set
%The dynamical system is interconnected with a static neural network based policy $u[t] = \pi(y[t])$.
%Remark: augment the system when the neural network policy depends on a finite impulse response length of the measurement $y$.

The goal of this paper is the following: \emph{Give a sufficient condition to ensure that $x[t]$, $u[t]$, $y[t]$ are within a pre-specified set for all $t \geq 0$ for any adversarial sequence $\{w[t]\}_{t=0}^\infty$ satisfying $w[t] \in \SigSp{W}, \forall t \geq 0$.} 

\textcolor{blue}{Be more specific: we are mostly working on weighted $\ell_{\infty}$ perturbation and certification. The plant $\tf{P}$ are mostly LTI.}
%Goal: verify the robustness, stability, constraint satisfaction for the neural network policy applied on the given plant


%The closed loop system is subject to an external perturbation $w$, which can be either adversarial or non-adversarial. Mathematically, the 

%When a neural network policy is interconnected with a dynamical system, the adversarial attack may cause the closed loop system to 
%In this paper, we analyze the impact of adversarial perturbation when a neural network policy is interconnected with a dynamical system. 
%The goal of this paper is to analyze the properties of a neural network when it is interconnected with a dynamical 

%\todo[inline]{Complete this part after Section 4. Add a block diagram}
%We consider a discrete time dynamical system with the following form:
% \begin{subequations}
% \begin{align}
% %x_{t+1} &= f(x_t, u_t, w_t) + \Delta_f(x_t, u_t, w_t) \label{eq:general1}\\
% %y_t &= g(x_t, u_t, w_t) + \Delta_g(x_t, u_t, w_t), \label{eq:general2}
% %x[t+1] &= f(x[t], u[t], w[t]) + \Delta_f(x[t], u[t], w[t]) \label{eq:general1}\\
% %y[t] &= g(x[t], u[t], w[t]) + \Delta_g(x[t], u[t], w[t]), \label{eq:general2}
% x[t+1] &= f(x[t], u[t], w[t]) + \Delta_f(x[1:t], u[1:t], w[1:t]) \label{eq:general1}\\
% y[t] &= g(x[t], w[t]), \label{eq:general2}
% \end{align}
% \end{subequations}

%Define the notation for vector and matrix
%Introduce the frequency domain notation: impulse response, z-transform, convolution, boldface symbol for signal and transfer matrix
%Define 
%Discrete time linear dynamical system in state space form
%Transfer matrix form: impulse response, z-transform, convolution
%Continuous time linear dynamical system in state space form
%Define absolute operator on a transfer matrix (absolutely summable, cite Munther and Mustafa's paper)



==> v1_3_linear.tex <==
In this section, we consider a special case of \eqref{eq:g1} - \eqref{eq:g5} in which the known dynamics $f$ and $g$ are linear time invariant (LTI) and the model uncertainty $\ttf{\Delta}$ is zero. The system dynamics are described by the following equations:
%We first specialize our discussion to a discrete time linear time invariant (LTI) system with no uncertainty
%We begin with the following discrete time linear time invariant (LTI) system
\begin{subequations}
\begin{align}
%x_{t+1} &= A x_t + B u_t + B_w w_t \label{eq:LTI1}\\
%y_t &= C x_t + D_w w_t, \label{eq:LTI2}
x[t+1] &= A x[t] + B u[t] + B_w w[t] \label{eq:LTI1}\\
y[t] &= C x[t] + D_w w[t], \label{eq:LTI2}\\
u[t] &= \pi(y[t]), \label{eq:LTI3}
\end{align}
\end{subequations}
%where $x$ is the state, $u$ the control action, $w$ the external disturbance. 
where $A$, $B$, $B_w$, $C$, and $D_w$ are matrices with appropriate dimensions and $\pi(\cdot)$ a neural network control policy.
%The system is interconnected with a static neural network based control policy $u[t] = \pi(y[t])$. %Without losing of generality, 
We consider the stabilization problem around $x = 0$ and assume that the pair $(A,B)$ is stabilizable and $(A,C)$ is detectable. The external disturbance $w$ can be either adversarial or non-adversarial. Note that the disturbance $w$ can affect both the neural network input $y$ and the system state $x$ (which includes the neural network output). We assume that $\tf w$ lies in a bounded space $\SigSp{W}$. 

In Section \ref{sec:open_stable}, we make the assumption that the system \eqref{eq:LTI1} - \eqref{eq:LTI2} is open loop stable, i.e., $\rho(A) < 1$. We derive a sufficient condition to ensure that the state and input constraints are satisfied under bounded adversarial attack $w \in \SigSp{W}$. We extend our results to unstable LTI systems in Section \ref{sec:open_unstable}. Finally, in Section \ref{sec:find_invariant}, we combine the results in Section \ref{sec:open_unstable} with the neural network certification tool and propose an algorithm to synthesize a certificate for satisfying the state and input constraints.

%guarantee closed loop boundedness under the assumption
%We assume that the system \eqref{eq:LTI1} - \eqref{eq:LTI2} is open loop stable, i.e., the spectral radius of the matrix $A$ is less than $1$.
%$A$ is Hurwitz, i.e., stable 
%(this implies that $(A,B_2)$ is stabilizable and $(A,C_2)$ is detectable). 
%($u$ and $y$ are also the delta's -- need to be justified)

\subsection{State and input constraints satisfaction for stable LTI systems} \label{sec:open_stable}
We use the frequency domain notation introduced in Section \ref{sec:notation} to analyze the property of the dynamical system \eqref{eq:LTI1} - \eqref{eq:LTI2}. Let $\tf{\Phi_{xu}} = (zI-A)^{-1} B$ and $\tf{\Phi_{xw}} = (zI-A)^{-1} B_w$ be the transfer matrices mapping from control $u$ and disturbance $w$ to state $x$, respectively. Similarly, let $\tf{\Phi_{yu}} = C (zI-A)^{-1} B$ and $\tf{\Phi_{yw}} = C (zI-A)^{-1} B_w + D_w$ be the transfer matrices mapping from control $u$ and disturbance $w$ to measurement $y$, respectively. Equations \eqref{eq:LTI1} - \eqref{eq:LTI2} can then be written in the frequency domain as
\begin{subequations}
\begin{align}
\tf x &= \tf{\Phi_{xw}} \tf w + \tf{\Phi_{xu}} \tf u \label{eq:LTIf1}\\
\tf y &= \tf{\Phi_{yw}} \tf w + \tf{\Phi_{yu}} \tf u. \label{eq:LTIf2}
\end{align}
\end{subequations}

% This may be confusing -- directly state
%\begin{theorem}
%Consider the system \eqref{eq:LTI1} - \eqref{eq:LTI2} with bounded disturbance $\tf w \in \SigSp{W}$. Suppose that we have $\tf u \in \SigSp{U}$ for all $\tf y \in \SigSp{Y}$ for the neural network policy $u = \pi(y)$ and the initial measurement $y_0 = C x_0 + D_w w_0$ is in the space $\SigSp{Y}$. If we have $\tf{\Phi_{yw}} \tf w + \tf{\Phi_{yu}} \tf u \in \SigSp{Y}$ for all $\tf w \in \SigSp{W}$ and $\tf u \in \SigSp{U}$, then the signals $\tf x$, $\tf y$ and $\tf u$ will be bounded.
%($\SigSp{U}, \SigSp{Y}$) forms an invariant set of the closed loop system. (bounded)
%the state constraint XXX is satisfied.
%\end{theorem}
%\begin{proof}
%The basic idea is to show that ($\SigSp{U}, \SigSp{Y}$) forms an invariant set of the closed loop system.
%a direct application of the invariant set principle
%\end{proof}
%\todo[inline]{Maybe move the proof to Appendix. Define positively invariant set of a dynamical system (cite Khalil's textbook) before the proof.}
%Definition of positively invariant set of a dynamical system (cite something, maybe Khalil's textbook)

In the following, we assume that the space $\SigSp{W}$ for the external disturbance is given by $\SigSp{W} = \{ \tf w \,\, | \,\, |w[t]| \preceq \bar{w}, \,\, \forall t \}$, where $\bar{w}$ is a vector with non-negative elements and $\preceq$ denotes the element-wise less than or equal to. For the neural network policy $u = \pi(y)$, we apply robustness analysis tool such as Fast-Lin to certify $|u| \preceq \bar{u}$ for all $|y| \preceq \bar{y}$. With these definitions, we can state the main theorem of this subsection:
%DeepPoly develops an algorithm to certify $|u[k]| \preceq U$ for all $|y[k]| \preceq Y$. Assume that the following constraint is satisfied:

\begin{theorem} \label{thm:LTI}
Consider a stable LTI system \eqref{eq:LTI1} - \eqref{eq:LTI2} with the neural network policy $u[t] = \pi(y[t])$. Assume that the adversarial perturbation is bounded in a set $|w[t]| \preceq \bar{w}$ for all $t \geq 0$. If we can find a pair of non-negative vectors $(\bar{y}, \bar{u})$ satisfying the following conditions:
\begin{enumerate}
    \item Neural network policy robustness certificate: The policy $u = \pi(y)$ has the property $|u| \preceq \bar{u}$ for all $|y| \preceq \bar{y}$
    \item Initial condition: $|y[0]| \preceq \bar{y}$
    \item Feedback condition: \text{abs}($\tf{\Phi_{yw}}$) $\bar{w}$ + \text{abs}($\tf{\Phi_{yu}}$) $\bar{u} \preceq \bar{y}$,
\end{enumerate}
then the following properties are satisfied:
\begin{enumerate}
    \item Bounded measurement and control: $|y[t]| \preceq \bar{y}$ and $|u[t]| \preceq \bar{u}$ for all $t \geq 0$
    \item Bounded state: $|x[t]| \preceq \text{abs}(\tf{\Phi_{xw}}) \bar{w} + \text{abs}(\tf{\Phi_{xu}}) \bar{u}$ for all $t \geq 0$
\end{enumerate}
\end{theorem}
% \begin{proof}
% We use mathematical induction to show that $\SigSp{I} = \{\begin{bmatrix} y \\ u \end{bmatrix} | \,\, |y| \preceq \bar{y}, |u| \preceq \bar{u}\}$ is a positively invariant set of the closed loop dynamical system. The first two conditions imply that $\begin{bmatrix} y[0] \\ u[0] \end{bmatrix} \in \SigSp{I}$. Assume that we have $\begin{bmatrix} y[t] \\ u[t] \end{bmatrix} \in \SigSp{I}$ for all $t < T$. From equation \eqref{eq:LTIf2}, we have
% \begin{subequations}
% \begin{align}
% |y[T]| &= |\sum_{\tau=0}^\infty \Phi_{yw}[\tau] w[T-\tau] + \Phi_{yu}[\tau] u[T-\tau] \, | \nonumber\\
% &\preceq \sum_{\tau=0}^\infty |\Phi_{yw}[\tau] w[T-\tau]| + |\Phi_{yu}[\tau] u[T-\tau] \, | \nonumber \\
% &\preceq \sum_{\tau=0}^\infty |\Phi_{yw}[\tau]| \bar{w} + |\Phi_{yu}[\tau]| \bar{u} \nonumber \\
% &= \text{abs}(\tf{\Phi_{yw}}) \bar{w} + \text{abs}(\tf{\Phi_{yu}}) \bar{u} \nonumber \\
% &\preceq \bar{y}
% \end{align}
% \end{subequations}
% where the last inequality is from the third condition. We then apply the first condition to obtain $|u[T]| \preceq \bar{u}$, and thus $\begin{bmatrix} y[T] \\ u[T] \end{bmatrix} \in \SigSp{I}$. Using mathematical induction, we conclude that $\begin{bmatrix} y[t] \\ u[t] \end{bmatrix} \in \SigSp{I}$ for all $t$.
% \end{proof}
%Assume the external disturbance $w$ is bounded at all time step $|w[k]| \preceq W$ ($\preceq$ denotes the element-wise less than or equal to). We define the absolute operator of a transfer matrix $\tf M$ as
%Define the element-wise $\ell_1$ norm of a transfer matrix $\tf M$ as
%\begin{equation}
%\text{abs}(\tf M) = \sum_{k=0}^\infty | M[k] |. \label{eq:element}
%\end{equation}
%We assume that each element of the transfer matrix $M$ is absolutely summable. (in Page 113 - 114 of the Signals and Systems textbook, stability is equivalent to absolutely summable / integrable for both discrete and continuous time)
%We only consider the case where the element-wise $\ell_1$ norm is bounded. Note that when $\tf M$ is FIR, its element-wise $\ell_1$ norm is always bounded.
%Then, $|u[k]| \preceq U$ and $|y[k]| \preceq Y$ forms an invariant set of the closed loop system. In this case, all the signal in the closed loop system are bounded.
\textcolor{blue}{Interpretation of Theorem \ref{thm:LTI}:} certificate on the boundedness of the closed loop system under adversarial attack (the notion of boundedness is weaker than the stability, as will be discussed later) We will discuss how to find a pair $(\bar{y}, \bar{u})$ satisfying the requirements in Section \ref{sec:find_invariant}.

%\begin{corollary}
%State constraint satisfaction: x in some set
%\end{corollary}

%Theorem \ref{thm:LTI} gives a
\textcolor{blue}{Discussion, need to be polished:}The major benefits of Theorem \ref{thm:LTI} is on its generality and simplicity. In particular, the theorem works for non-differentiable or even discontinuous neural network policy $\pi(\cdot)$, as long as we can derive the property $|u| \preceq \bar{u}$ for all $|y| \preceq \bar{y}$. Many popular neural networks exhibit non-differentiability or discontinuity, due to either quantization, digitalization, switching behavior, obfuscated gradient, or many other defense strategies. In addition, some non-neural network policies such as decision tree and random forest are discontinuous in nature. The stability of non-differentiable or discontinuous policy in the loop are usually not treated in the existing literature. On the other hand, Theorem \ref{thm:LTI} gives a simple algebraic (linear programming) test to certify the closed loop boundedness of non-differentiable or discontinuous policy in the loop, as long as certain technical property of the policy can be derived. Even for differentiable neural network policy, this approach can prove boundedness for a larger class of policy than the Lipschitz-based stability certification method.

%\textbf{Pros:} 
%\begin{enumerate}
%    \item This method is a simple algebraic (LP) test
%    \item Work for non-continuous neural network policy (switch), discontinuous (quantization, digitalization)
%    \item Even for continuous neural network policy, this approach can prove stability for a larger class of policy than the Lipchitz-based stability certification 
%    \item We already have tools (DeepPoly,...etc) to calculate the input and output sets
%\end{enumerate}
%\textbf{Cons:}
%\begin{enumerate}
%    \item This notion of stability is weaker than input-output stability, Lyapunov stability, and asymptotic stability because we cannot guarantee we can approach the equilibrium point as close as possible. In particular, we cannot show that the state deviation $x$ goes to zero when the external disturbance $w$ is zero.
%    \item We need to try the invariant set $U$ and $Y$.
%\end{enumerate}

We note that when the neural network policy has stronger technical conditions such as Lipschitz continuous with finite $\mathcal{L}_2$ gain, i.e., $\| \tf u \|_{\ell_2} \leq \gamma \|\tf y \|_{\ell_2}$ for some finite $\gamma$, we can use the idea similar to Theorem \ref{thm:LTI} to show the input-output stability of the closed loop system. We say that the closed loop system is input-output stable if the gain from adversarial perturbation $\tf w$ to the output $\tf y$ is finite. If we use the $\ell_2$ norm to characterize the magnitude of the signals $\tf w$ and $\tf y$, then we have the following result: 
%To show stronger stability guarantee, we need to get the local Lipschitz constant of the region. Specifically, to show that the closed loop system is input-output stable with finite gain, we need the neural network itself to have finite input output gain. For instance, 
\begin{theorem} \label{lemma:Hinf}
Suppose that the neural network policy $u = \pi(y)$ has a finite $\mathcal{L}_2$ gain $\gamma$, i.e., $\| \tf u \|_{\ell_2} \leq \gamma \|\tf y \|_{\ell_2}$. If $\|\tf{\Phi_{yu}}\|_{\mathcal{H}_\infty} < \frac{1}{\gamma}$, then the closed loop system is input-output stable. 
%$\ell_2$ induced norm and $\mathcal{H}_\infty$, small gain theorem for stability
\end{theorem}
% \begin{proof}
% This is a direct application of the small gain theorem \cite{zhou1996robust}. We have
% \begin{subequations}
% \begin{align}
% \| \tf y \|_{\ell_2} &= \| \tf{\Phi_{yw}} \tf w + \tf{\Phi_{yu}} \tf u \|_{\ell_2} \label{eq:small1}\\
% &\leq \| \tf{\Phi_{yw}} \tf w \|_{\ell_2} + \|\tf{\Phi_{yu}} \tf u \|_{\ell_2} \label{eq:small2} \\
% &\leq \| \tf{\Phi_{yw}}\|_{\mathcal{H}_\infty} \|\tf w \|_{\ell_2} + \|\tf{\Phi_{yu}} \|_{\mathcal{H}_\infty} \|\tf u \|_{\ell_2} \label{eq:small3} \\
% & \leq \| \tf{\Phi_{yw}}\|_{\mathcal{H}_\infty} \|\tf w \|_{\ell_2} + \|\tf{\Phi_{yu}} \|_{\mathcal{H}_\infty} \gamma \|\tf y \|_{\ell_2}. \label{eq:small4}
% \end{align}
% \end{subequations}
% where \eqref{eq:small2} comes from the subadditivity property of a norm and \eqref{eq:small3} from the fact that $\mathcal{H}_\infty$ norm is equivalent to the $\ell_2$ to $\ell_2$ induced norm. By assumption, we have $\|\tf{\Phi_{yu}}\|_{\mathcal{H}_\infty} \gamma < 1$. Therefore, we have
% \begin{equation}
% \| \tf y \|_{\ell_2} \leq (1 - \gamma \|\tf{\Phi_{yu}}\|_{\mathcal{H}_\infty})^{-1} \| \tf{\Phi_{yw}}\|_{\mathcal{H}_\infty} \|\tf w \|_{\ell_2},
% \end{equation}
% which means that the $\mathcal{L}_2$ gain from input $\tf w$ to output $\tf y$ is bounded. This implies input-output stability of the closed loop system.
% \end{proof}
The above theorem is a direct consequence of the small gain theorem \cite{zhou1996robust} and the fact that the $\mathcal{H}_\infty$ norm of a system is equivalent to the $\ell_2$ to $\ell_2$ induced norm. Note that when the magnitude of the adversarial perturbation $\tf w$ tends to $0$, the above theorem implies that the magnitude of the neural network input $\tf y$ and the control action $\tf u$ will also go to $0$. By the assumption that the pair $(A,C)$ is detectable, this further implies that $x = 0$ is a stable equilibrium. 

When the magnitude of the signals $\tf w$ and $\tf y$ is characterized by the $\ell_\infty$ norm, we can replace the $\mathcal{H}_\infty$ norm with the $\mathcal{L}_1$ system norm \cite{dahleh19871} in Theorem \ref{lemma:Hinf}. The $\mathcal{L}_1$ norm \cite{dahleh19871} of a transfer matrix is defined as
\begin{equation}
    \|\tf{G}\|_{\mathcal{L}_1} = \underset{i}{\text{max}} \sum_{j=1}^n \|\tf{g_{ij}}\|_1 = \underset{i}{\text{max}} \sum_{j=1}^n \sum_{t=0}^\infty |g_{ij}[t]| \nonumber
\end{equation}
where $\tf{g_{ij}}$ is the $(i,j)$-th entry of the transfer matrix $\tf{G}$ and $n$ is the number of column of $\tf{G}$. The $\mathcal{L}_1$ norm of a system is equivalent to the $\ell_\infty$ to $\ell_\infty$ induced norm \cite{dahleh19871}. We then have the following corollary of Theorem \ref{lemma:Hinf}:
\begin{corollary} \label{lemma:L1}
Suppose that the neural network policy $u = \pi(y)$ has a finite $\ell_\infty$ to $\ell_\infty$ gain $\gamma$, i.e., $\| \tf u \|_{\ell_\infty} \leq \gamma \|\tf y \|_{\ell_\infty}$. If $\|\tf{\Phi_{yu}}\|_{\mathcal{L}_1} < \frac{1}{\gamma}$, then the closed loop system is input-output stable. 
%$\ell_2$ induced norm and $\mathcal{H}_\infty$, small gain theorem for stability
\end{corollary}

% \begin{corollary}
% $\ell_\infty$ to $\ell_\infty$ induced norm corresponds to $\mathcal{L}_1$ system norm \cite{dahleh19871}
% \end{corollary}

\subsection{Unstable LTI systems} \label{sec:open_unstable}
In this subsection, we consider the case where the open loop system \eqref{eq:LTI1} - \eqref{eq:LTI2} is unstable. Our strategy is to extract a first order approximation of the control policy to stabilize the plant first, then analyze the interconnection of the stabilized plant and the residual control policy. Specifically, we rewrite the neural network policy as $u[t] = \pi(y[t]) = K_0 y[t] + \pi_0(y[t])$ for some matrix $K_0$. We call $\pi_0(\cdot)$ the residual control policy. Equations \eqref{eq:LTI1} - \eqref{eq:LTI3} then become
\begin{subequations}
\begin{align}
x[t+1] &= (A + B K_0 C) x[t] + B u_0[t] + (B K_0 D_w + B_w) w[t] \label{eq:LLTI1}\\
y[t] &= C x[t] + D_w w[t] \label{eq:LLTI2} \\
u_0[t] &= \pi_0(y[t]). \label{eq:LLTI3}
\end{align}
\end{subequations}
As long as the spectral radius of the closed loop system matrix $A_{cl} = (A + B K_0 C)$ is less than $1$, the transfer matrix $(zI - A_{cl})^{-1}$ is stable. Theorem \ref{thm:LTI} can then be used with redefined transfer matrices $\tf{\Phi_{xu}} = (zI-A_{cl})^{-1} B$, $\tf{\Phi_{xw}} = (zI-A_{cl})^{-1} (B K_0 D_w + B_w)$, $\tf{\Phi_{yu}} = C \tf{\Phi_{xu}}$, and $\tf{\Phi_{yw}} = C \tf{\Phi_{xw}} + D_w$. In the following, we propose two different ways to obtain a candidate $K_0$: (1) using the Jacobian evaluated at the origin, and (2) using neural network certification tool to find a first order approximation of the policy over a region.

\subsubsection{Obtaining $K_0$ using Jacobian}
If the neural network policy has the property $\pi(0) = 0$ and is differentiable at $y = 0$, we can use the Jacobian of $\pi(y)$ evaluated at $y = 0$ as a candidate for $K_0$, i.e., $K_0 = \frac{\partial \pi(y)}{\partial y}\Bigr|_{y=0}$. In this case, the residual control policy $\pi_0(y)$ has the following property:
\begin{equation}
    \pi_0(0) = 0, \quad \underset{\|y\| \to 0}{\text{limit}} \,\, \frac{\|\pi_0(y)\|}{\|y\|} \to 0 \label{eq:res_cont}%\,\, \text{as} \,\, \|y\| \to 0. 
\end{equation}
We then have the following Lemma directly adopt from Theorem $4.3$ in \cite{astrom2010feedback}.
\begin{lemma}[Local stability] \label{lemma:local}
Consider the dynamical system \eqref{eq:LLTI1} - \eqref{eq:LLTI3} with the residual control policy $\pi_0(y) = \pi(y) - K_0 y$ satisfying \eqref{eq:res_cont}. If $\rho(A + B K_0 C) < 1$, then $x = 0$ is a locally asymptotically stable equilibrium point of the system \eqref{eq:LLTI1} - \eqref{eq:LLTI3}. On the other hand, if $\rho(A + B K_0 C) > 1$, then $x = 0$ is a locally unstable equilibrium point of the system \eqref{eq:LLTI1} - \eqref{eq:LLTI3}.
\end{lemma}

Note that the conditions for Lemma \ref{lemma:local} can be strict for many neural networks. As will be shown in Section \ref{sec:experiment}, many neural networks trained by reinforcement learning algorithms such as DDPG, TRPO, and PPO can obtain perfect rewards in certain task, but the policies are indeed locally \emph{unstable} according to the conditions from Lemma \ref{lemma:local}. This is because we do not explicitly incorporate the stability as a requirement into the reward function. For these neural networks, one cannot use the stability analysis methods proposed in \cite{berkenkamp2017safe}, \cite{jin2018stability}, \cite{jin2018control}, \cite{richards2018lyapunov} to show that the state and input constraints are satisfied because a stable equilibrium does not exist. On the other hand, Theorem \ref{thm:LTI} is still a valid sufficient condition to certify that the state and input constraints are satisfied even when a stable equilibrium does not exist.

\subsubsection{Obtaining $K_0$ using neural network certification tools}
If the neural network policy is not differentiable or the equilibrium $x = 0$ are shown to be locally unstable according to Lemma \ref{lemma:local}, one can use the neural network certification tools to find a different candidate $K_0$. For instance, Fast-Lin, CROWN, and CNN-cert provide a pair of linear lower and upper bounds on the neural network output as
\begin{equation}
    K_L y + b_L \leq \pi(y) \leq K_U + b_U, \quad \forall | y | \preceq y_{ref}. \label{eq:NN-CERT}
\end{equation}
A candidate $K_0$ is given by $(K_U + K_L)/2$, which is a first order approximation of the control policy over a region. Based on our observation, the $K_0$ found by this method is more likely to make the system matrix $A_{cl} = (A + B K_0 C)$ stable as it is less sensitive to the input than the gradient. As long as we can find a $K_0$ to make $\rho(A_{cl}) < 1$, we can apply Theorem \ref{thm:LTI} to check if the input and state constraints can be satisfied under the bounded adversarial perturbation. 

%Conceptually, $(A_U + A_L)/2$ captures the trend of gradient over a region. 
%we can use Fast-Lin to extract a first order approximation of the control policy.

\subsection{Finding a certified invariant set} \label{sec:find_invariant}
In this subsection, we propose a simple iterative algorithm to synthesize a pair of vectors $(\bar{u}, \bar{y})$ satisfying the conditions in Theorem \ref{thm:LTI}. We assume that a matrix $K_d$ with $\rho(A + B K_d C) < 1$ is given as a default linear approximation of the neural network policy\footnote{We note that finding a static gain $K$ to make $(A + B K C)$ a stable matrix is known as the static output feedback problem in the control literature. In the worst case, this problem can be NP-hard \cite{blondel1997np}. For an output feedback problem, one may consider using a dynamic (recurrent) policy for control, but that is beyond the scope of this paper.}. For the ease of presentation, we assume that the initial condition $x[0]$ is $0$ so the second condition of Theorem \ref{thm:LTI} is implied by the third condition. The algorithm is summarized in Algorithm \ref{alg:lin}.

\input{_Algo_linear.tex}

%show how to certify the closed loop boundedness of a given test set $(\bar{u}, \bar{y})$. 
Algorithm \ref{alg:lin} can be interpreted as follows. We calculate the bounds for $\bar{u}$ and $\bar{u_0}$ over the region $|y| \preceq y_{ref}$ using the neural network certification tool from Lines $4$ to $11$. We also extract a linear policy $K$ to make the closed loop transfer matrices stable. Given the range of the adversarial perturbation $\bar{w}$ and the residual control action $\bar{u_0}$, we calculate the bounds for the state $x$ and the measurement $y$. If the condition $\bar{y} \preceq y_{ref}$ is satisfied, then we have $|y[t]| \preceq \bar{y}$ and $|u[t]| \preceq \bar{u}$ for all $t \geq 0$ according to Theorem \ref{thm:LTI}, which gives a certificate for closed loop boundedness. If $\bar{y} \not\preceq y_{ref}$, we then increase the test bound $y_{ref}$ and repeat the search. 

%We start with a test bound $y_{ref} = 0$ and calculate the approximate linear policy of the neural network 
%Idea: start with $\bar{y}^{(0)} = (1+\epsilon)$ abs($\tf{\Phi_{yw}}$) $\bar{w}$. Derive $\bar{u}^{0}$ using the certification tool. Test $\bar{y}^{(k+1)} = (1+\epsilon)$ [abs($\tf{\Phi_{yw}}$) $\bar{w}$ + abs($\tf{\Phi_{yu}}$) $\bar{u}^{(k)}$] until converges. If converges, then we get a certificate

==> v1_4_nonlinear.tex <==
%Bascially just include all the nonlinearity in a delta block
In this section, we consider the general form of the system shown in Figure \ref{fig:model}.
% \begin{subequations}
% \begin{align}
% x[t+1] &= f(x[t], u[t], w[t], \delta[t]) \label{eq:g1}\\
% y[t] &= g(x[t], w[t]) \label{eq:g2} \\
% \alpha[t] &= h(x[t], u[t], w[t]) \label{eq:g3} \\
% u[t] &= \pi(y[t]) \label{eq:g4} \\
% \ttf{\delta} = \Delta(\ttf{\alpha}) \label{eq:g5}.
% \end{align}
% \end{subequations}
% %with the neural network policy $u[t] = \pi(y[t])$ and the uncertainty-induced input $\ttf{\delta} = \Delta(\ttf{\alpha})$. 
% We assume $y$ in \eqref{eq:g2} is not a direct function of $u$ and $\delta$, and $\alpha$ in \eqref{eq:g3} is not a direct function of $\delta$. This assumption is to ensure the well-posedness of the feedback structure in Fig. XXX (no algebraic loop).

\subsection{Linearization}
We first linearize the system \eqref{eq:g1} - \eqref{eq:g3} around $0$ as
\begin{subequations}
\begin{align}
%x_{t+1} &= A x_t + B u_t + B_w w_t \label{eq:LTI1}\\
%y_t &= C x_t + D_w w_t, \label{eq:LTI2}
x[t+1] &= A x[t] + B u[t] + B_w w[t] + B_{\delta} \delta[t] \label{eq:NLTI1}\\
y[t] &= C x[t] + D_w w[t] \label{eq:NLTI2} \\
\alpha[t] &= C_{\alpha} x[t] + D_{\alpha u} u[t] + D_{\alpha w} w[t]. \label{eq:NLTI3}
\end{align}
\end{subequations}
with
\begin{subequations}
\begin{align}
A &= \frac{\partial f}{\partial x}\Bigr|_{x=0}, \quad B = \frac{\partial f}{\partial u}\Bigr|_{u=0}, \quad B_w = \frac{\partial f}{\partial w}\Bigr|_{w=0}, \quad B_\delta = \frac{\partial f}{\partial \delta}\Bigr|_{\delta=0} \nonumber\\
C &= \frac{\partial g}{\partial x}\Bigr|_{x=0}, \quad D_w = \frac{\partial g}{\partial w}\Bigr|_{w=0}, \quad C_\alpha = \frac{\partial h}{\partial x}\Bigr|_{x=0}, \quad D_{\alpha u} = \frac{\partial h}{\partial u}\Bigr|_{u=0}, \quad D_{\alpha w} = \frac{\partial h}{\partial w}\Bigr|_{w=0}. \nonumber
\end{align}
\end{subequations}
We absorb all the linearization-induced uncertainty into either the external perturbation $w$ or the model uncertainty block $\Delta$. This part will be discussed in more details in the next subsecction. \textcolor{blue}{A needs to be stable, use the technique from Section \ref{sec:open_unstable}}
%Linearize the known nonlinear dynamic and absorb the linearization-induced uncertainty into the original uncertain dynamic term. 
%The control policy is a static neural network $u[t] = \pi(y[t])$, and the uncertain input $\delta$ is calculated by $\ttf{\delta} = \Delta(\ttf{\alpha})$, which can be dynamic. 
Similar to the previous section, we rewrite \eqref{eq:NLTI1} - \eqref{eq:NLTI3} in the frequency domain as
\begin{subequations}
\begin{align}
\tf{x} &= \tf{\Phi_{xu}} \tf u + \tf{\Phi_{xw}} \tf w + \tf{\Phi_{x\delta}} \ttf{\delta} \label{eq:FNLTI1}\\
\tf{y} &= \tf{\Phi_{yu}} \tf u + \tf{\Phi_{yw}} \tf w + \tf{\Phi_{y\delta}} \ttf{\delta} \label{eq:FNLTI2}\\
\ttf{\alpha} &= \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w + \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \ttf{\delta} \label{eq:FNLTI3}
\end{align}
\end{subequations}
with $\tf{\Phi_{xu}} = (zI-A)^{-1} B$, $\tf{\Phi_{xw}} = (zI-A)^{-1} B_w$, $\tf{\Phi_{x \ttf{\delta}}} = (zI-A)^{-1} B_\delta$, $\tf{\Phi_{yu}} = C (zI-A)^{-1} B$, $\tf{\Phi_{yw}} = C (zI-A)^{-1} B_w + D_w$, $\tf{\Phi_{y \ttf{\delta}}} = C(zI-A)^{-1} B_\delta$, $\tf{\Phi_{\alpha u}} = C_{\alpha}(zI-A)^{-1} B + D_{\ttf{\alpha} u}$, $\tf{\Phi_{\ttf{\alpha} w}} = C_{\alpha}(zI-A)^{-1} B_w + D_{\alpha w}$, and $\tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} = C_{\alpha}(zI-A)^{-1} B_\delta$. The following theorem is a straightforward extension of Theorem \ref{thm:LTI}. 
\begin{theorem} \label{thm:NLTI}
Consider the plant \eqref{eq:NLTI1} - \eqref{eq:NLTI2} with the neural network policy $u[t] = \pi(y[t])$ and the uncertainty $\ttf{\delta} = \Delta(\ttf{\alpha})$. Assume that the adversarial perturbation is bounded in a set $|w[t]| \preceq \bar{w}$ for all $t \geq 0$. If we can find a quadruplet $(\bar{y}, \bar{u}, \bar{\delta}, \bar{\alpha})$ satisfy the following conditions:
\begin{enumerate}
    \item Neural network policy robustness certificate: The policy $u = \pi(y)$ has the property $|u| \preceq \bar{u}$ for all $|y| \preceq \bar{y}$
    \item Input-output relation of the uncertainty block: $\ttf{\delta} = \Delta(\ttf{\alpha})$ has the property $| \alpha[k] | \preceq \bar{\alpha}$, $k = 0, \cdots, t$ $\implies$ $| \delta[t] | \preceq \bar{\delta}$ for all $t \geq 0$.
    \item Initial condition: $|y[0]| \preceq \bar{y}$, $|\alpha[0]| \preceq \bar{\alpha}$
    \item Feedback condition: \text{abs}($\tf{\Phi_{yw}}$) $\bar{w}$ + \text{abs}($\tf{\Phi_{yu}}$) $\bar{u}$ + \text{abs}($\tf{\Phi_{y\ttf{\delta}}}$) $\bar{\delta}$ $\preceq \bar{y}$ and \text{abs}($\tf{\Phi_{\ttf{\alpha}w}}$) $\bar{w}$ + \text{abs}($\tf{\Phi_{\ttf{\alpha}u}}$) $\bar{u}$ + \text{abs}($\tf{\Phi_{\ttf{\alpha} \ttf{\delta}}}$) $\bar{\delta}$ $\preceq \bar{\alpha}$
\end{enumerate}
then we have the following properties:
\begin{enumerate}
    \item Bounded feedback signals: $|y[t]| \preceq \bar{y}$, $|u[t]| \preceq \bar{u}$, $|\alpha[t]| \preceq \bar{\alpha}$, $|\delta[t]| \preceq \bar{\delta}$ for all $t \geq 0$
    \item Bounded state: $|x[t]| \preceq$ \text{abs}($\tf{\Phi_{xw}}$) $\bar{w}$ + \text{abs}($\tf{\Phi_{xu}}$) $\bar{u}$ + \text{abs}($\tf{\Phi_{x\ttf{\delta}}}$) $\bar{\delta}$ for all $t \geq 0$
\end{enumerate}
\end{theorem}

%\todo[inline]{Study structured singular value and D-K iteration. Derive the $\mathcal{L}_1$ version and the $\mathcal{H}_\infty$ version for stability.}
% Without losing generality, we assume $\| \Delta \|_{\mathcal{L}_1} \leq 1$. With this assumption, we always have $\| \ttf{\delta} \|_{\ell_\infty} \leq \| \ttf{\alpha} \|_{\ell_\infty}$. To show stability, we first require $\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1} < 1$ so that the loop between the plant and the uncertainty $\tf{\Delta}$ is stable. We then have
% \begin{subequations}
% \begin{align}
% \| \ttf{\delta} \|_{\ell_\infty} & \leq \| \ttf{\alpha} \|_{\ell_\infty} \nonumber\\
% &= \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w + \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \ttf{\delta} \|_{\ell_\infty} \nonumber\\
% &\leq \| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1} \| \ttf{\delta} \|_{\ell_\infty} + \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w \|_{\ell_\infty}.
% \end{align}
% \end{subequations}
% From the assumption $\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1} < 1$, we have
% \begin{equation}
% \| \ttf{\delta} \|_{\ell_\infty} \leq (1-\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1})^{-1} \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w \|_{\ell_\infty}    
% \end{equation}
% Then, we have
% \begin{subequations}
% \begin{align}
% \| \tf y \|_{\ell_\infty} & \leq \| \tf{\Phi_{y \ttf{\delta}}}\|_{\mathcal{L}_1} \|\ttf{\delta}\|_{\ell_\infty} + \| \tf{\Phi_{yu}} \tf u + \tf{\Phi_{yw}} \tf w\|_{\ell_\infty} \nonumber\\
% &\leq \| \tf{\Phi_{y \ttf{\delta}}}\|_{\mathcal{L}_1} (1-\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1})^{-1} \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w \|_{\ell_\infty} + \| \tf{\Phi_{yu}} \tf u + \tf{\Phi_{yw}} \tf w\|_{\ell_\infty}
% \end{align}
% \end{subequations}

\subsection{Bounds for the linearization error over a region}
In order to certify that the state constraints are satisfied when the neural network policy is interconnected with the nonlinear model, we need to bound the linearization error as part of the uncertainty block. 

\subsection{Algorithm}


==> v1_5_Experiments.tex <==
%\todo[inline]{What examples are we going to show here?}
%We need a killer example here...
%MuJoCo

% Simple classical control: Inverted pendulum, double inverted pendulum, quadruple inverted pendulum
% \begin{enumerate}
%     \item Code the physics-based simulator: discretize the continuous time nonlinear equation
%     \item Assume that the physics parameters are partially known -- model the uncertainty set
%     \item Linearize the dynamic with nonlinear equation
%     \item Train a neural network policy for stabilization -- consider using both deep deterministic policy gradient (DDPG) and DQN (discontinuous control strategy)
%     \item Neural network robustness certification
%     \item Find closed loop invariant set, prove robust stability (check how to calculate the $\mathcal{H}_\infty$ and the $\mathcal{L}_1$ norms).
%     \item Demonstrate adversarial attack 
% \end{enumerate}

Test different NN certification algorithm (from exact solution to approximated solution)
Compare the tightness of the invariant set based method vs Lipschitz based method.
Expected result: the invariant set based method is tighter because we tend to over-estimate the Lipschitz constant.

May need to compare with other people's method

%More advanced example (with image classifier in between): how do we derive the plant model in this case?

\subsection{System model}

\subsection{Training of a neural network policy}

\subsection{Certification with the linearized dynamics}

\subsection{Certification with the nonlinear dynamics}




==> v1_Algo_linear.tex <==
\begin{algorithm}[ht]
   \caption{Certification of state and input constraints for LTI systems}
   \label{alg:lin}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:}  Constraint limits $x_{lim}$, $y_{lim}$, $u_{lim}$, adversarial perturbation bound $\bar{w}$, initial bound $y_{ref} = 0$, default approximation $K_d$, parameter $\epsilon > 0$, flag Success = False, Done = False, all system matrices in \eqref{eq:LTI1} - \eqref{eq:LTI3}
   \STATE {\bfseries Output:} flag Success, certified bounds $\bar{x}$, $\bar{y}$, $\bar{u}$
   %\REPEAT
   \WHILE{Done == False}
   \STATE $K_L$, $b_L$, $K_U$, $b_U$ = NN-CERT($\pi$, $y_{ref}$) from equation \eqref{eq:NN-CERT}
   \STATE $K = (K_L + K_U)/2$
   \IF{$\rho(A + B K C) > 0.995$}
   \STATE $K = K_d$  %// use default $K_d$
   \ENDIF
   \STATE $A_{cl} = A + B K C$
   \STATE $\bar{u} =$ max($|K_L| y_{ref} + |b_L|$, $|K_U| y_{ref} + |b_U|$)
   \STATE $\bar{u_0} =$ max($|K_L - K| y_{ref} + |b_L|$, $|K_U - K| y_{ref} + |b_U|$)
   \STATE Calculate the transfer matrices $\tf{\Phi_{xu}}, \tf{\Phi_{xw}}, \tf{\Phi_{yu}}, \tf{\Phi_{yw}}$
   \STATE $\bar{x} =$ abs($\tf{\Phi_{xw}}$) $\bar{w}$ + abs($\tf{\Phi_{xu}}$) $\bar{u_0}$
   \STATE $\bar{y} =$ abs($\tf{\Phi_{yw}}$) $\bar{w}$ + abs($\tf{\Phi_{yu}}$) $\bar{u_0}$
   \IF {$\bar{x} \not \preceq x_{lim}$ or $\bar{y} \not \preceq y_{lim}$ or $\bar{u} \not \preceq u_{lim}$}
   \STATE Done = True
   \ELSIF {$\bar{y} \preceq y_{ref}$}
   \STATE Success = True, Done = True
   \ELSE
   \STATE $y_{ref} = (1+\epsilon) \bar{y}$
   \ENDIF
   \ENDWHILE
   \STATE \textbf{Return} Success, $\bar{x}$, $\bar{y}$, $\bar{u}$
\end{algorithmic}
\end{algorithm}

==> v1_App_CartPole.tex <==
Let $\eta$ be the displacement of the cart and $\theta$ be the angle of the pole. The dynamics of the cart pole is given by
\begin{subequations}
\begin{align}
\Ddot{\eta} &= M_t^{-1} (\frac{4}{3}ml^2 \dot{\theta}^2 \text{sin}(\theta) - mgl\text{sin}(\theta)\text{cos}(\theta) - \frac{4}{3}lb\dot{\eta} + \frac{4}{3}lu )\nonumber\\
\Ddot{\theta} &= M_t^{-1}(-ml\dot{\theta}^2\text{sin}(\theta)\text{cos}(\theta) + (M+m)g\text{sin}(\theta) + \text{cos}(\theta) b\dot{\eta} - \text{cos}(\theta)u) \nonumber
\end{align}\label{eq:nonlinear_cont}
\end{subequations}
with
\begin{equation}
    M_t = \frac{4}{3}(M+m)l - ml \text{cos}^2(\theta)
\end{equation}

Using Euler discretization, the nonlinear discrete time cart pole model is given by
\begin{subequations}
\begin{align}
\eta[t+1] &= \eta[t] + \tau \dot{\eta}[t] \nonumber\\
\dot{\eta}[t+1] &= \dot{\eta}[t] + \tau \Ddot{\eta}[t] \nonumber\\
\theta[t+1] &= \theta[t] + \tau \dot{\theta}[t] \nonumber\\
\dot{\theta}[t+1] &= \dot{\theta}[t] + \tau \Ddot{\theta}[t] \nonumber
\end{align}\label{eq:nonlinear_disc}
\end{subequations}
with sampling time $\tau$. Define the state vector $x = \begin{bmatrix} \eta & \dot{\eta} & \theta & \dot{\theta}\end{bmatrix}^\top$. The linearization of \eqref{eq:nonlinear_disc} around the origin is given by $x[t+1] = A x[t] + B u[t]$ with
\begin{equation}
A = \begin{bmatrix}1 & \tau & 0 & 0 \\ 0 & 1 - \frac{4\tau b}{4M+m} & \frac{-3mg\tau}{4M+m} & 0 \\ 0 & 0 & 1 & \tau \\ 0 & \frac{3\tau b}{(4M+m)l} & \frac{3(M+m)g\tau}{(4M+m)l} & 1\end{bmatrix}, \quad B = \begin{bmatrix} 0 \\ \frac{4\tau}{4M+m} \\ 0 \\ \frac{-3\tau}{(4M+m)l}\end{bmatrix} \label{eq:linear_disc}
\end{equation}

The linearization of the model induces some mismatch between \eqref{eq:nonlinear_disc} and \eqref{eq:linear_disc}. In the following, we derive a bound on the linearization error and model it as an uncertainty block. We first assume that the original nonlinear model can be written as $x[t+1] = A x[t] + B u[t] + \delta[t]$ with $\delta[t]$ being the linearization error. We note that $\delta[t]$ has the following sparsity structure
\begin{equation}
    \delta[t] = \begin{bmatrix} 0 \\ \delta_\eta[t] \\ 0 \\ \delta_\theta[t] \end{bmatrix}. \nonumber
\end{equation}
We assume that the state vector is bounded by the constraint
\begin{equation}
    | \begin{bmatrix}\eta \\ \dot{\eta} \\ \theta \\ \dot{\theta}\end{bmatrix} | \leq \begin{bmatrix}\bar{\eta} \\ \bar{\dot{\eta}} \\ \bar{\theta} \\ \bar{\dot{\theta}}\end{bmatrix}
\end{equation}
at all time $t$. Our goal is to bound the range of $\delta_\eta[t]$ and $\delta_\theta[t]$.

An exact formulation of $\delta_\eta[t]$ and $\delta_\theta[t]$ is given by
\begin{subequations}
\begin{align}
\delta_\eta &= \frac{\tau}{M_a} \Big[ 12m\text{sin}^2(\theta)(b\dot{\eta} - u) + (4M+m)(4ml\dot{\theta}^2 - 3mg\text{cos}(\theta))\text{sin}(\theta) + 3mg\theta(4M+m+3m\text{sin}^2(\theta)) \Big]\nonumber\\
\delta_\theta &= \frac{\tau}{M_a l}\Big[ 3(u - b\dot{\eta})((4M+m)(1-\text{cos}(\theta)) + 3m\text{sin}^2(\theta)) + 3(4M+m)\text{sin}(\theta)((M+m)g - ml\dot{\theta}^2\text{cos}(\theta)) \nonumber\\
& -3(4M+m+3m\text{sin}^2(\theta))(M+m)g\theta\Big]\nonumber\\
M_a &= (4M + m)(4M + m + 3m\text{sin}^2(\theta)) \nonumber
\end{align}\label{eq:err_disc}
\end{subequations}

Note that for $0 \leq \theta \leq \pi$, we have $\theta \geq$ sin($\theta$) $\geq \theta(1 - \frac{\theta}{\pi})$. We then have
\begin{subequations}
\begin{align}
| \delta_\eta | &\leq \tau \Big[ |\frac{12m\text{sin}^2(\bar{\theta})}{(4M+m)^2}| |u - b\dot{\eta}| + |\frac{6mg\bar{\theta}}{(4M+m)\pi} + \frac{9m^2 g\text{sin}^2(\bar{\theta})}{(4M+m)^2}| |\theta| + |\frac{4ml\text{sin}(\bar{\theta})\bar{\dot{\theta}}}{4M+m}| |\dot{\theta}| \Big] \nonumber\\
| \delta_\theta | &\leq \tau \Big[ |\frac{3(1-\text{cos}(\bar{\theta}))}{(4M+m)l} + \frac{3m\text{sin}^2(\bar{\theta})}{(4M+m)^2 l}| |u - b\dot{\eta}| + |\frac{3(M+m)g\bar{\theta}}{(4M+m)l\pi} + \frac{9m(M+m)g\text{sin}^2(\bar{\theta})}{(4M+m)^2 l}| |\theta| \nonumber\\
& + |\frac{1.5m\text{sin}(2\bar{\theta})\bar{\dot{\theta}}}{4M+m}| |\dot{\theta}| \Big] \nonumber
\end{align}\label{eq:err_bnd}
\end{subequations}

==> v1_App_proof_thm1.tex <==
The proof of Theorem \ref{thm:LTI} relies on the concept of positively invariant set, which is defined as follows:
\todo[inline]{Define positively invariant set of a dynamical system (cite Khalil's textbook) before the proof.}

\begin{proof}[Proof of Theorem \ref{thm:LTI}]
We use mathematical induction to show that $\SigSp{I} = \{\begin{bmatrix} y \\ u \end{bmatrix} | \,\, |y| \preceq \bar{y}, |u| \preceq \bar{u}\}$ is a positively invariant set of the closed loop dynamical system. The first two conditions imply that $\begin{bmatrix} y[0] \\ u[0] \end{bmatrix} \in \SigSp{I}$. Assume that we have $\begin{bmatrix} y[t] \\ u[t] \end{bmatrix} \in \SigSp{I}$ for all $t < T$. From equation \eqref{eq:LTIf2}, we have
\begin{subequations}
\begin{align}
|y[T]| &= |\sum_{\tau=0}^\infty \Phi_{yw}[\tau] w[T-\tau] + \Phi_{yu}[\tau] u[T-\tau] \, | \nonumber\\
&\preceq \sum_{\tau=0}^\infty |\Phi_{yw}[\tau] w[T-\tau]| + |\Phi_{yu}[\tau] u[T-\tau] \, | \nonumber \\
&\preceq \sum_{\tau=0}^\infty |\Phi_{yw}[\tau]| \bar{w} + |\Phi_{yu}[\tau]| \bar{u} \nonumber \\
&= \text{abs}(\tf{\Phi_{yw}}) \bar{w} + \text{abs}(\tf{\Phi_{yu}}) \bar{u} \nonumber \\
&\preceq \bar{y}
\end{align}
\end{subequations}
where the last inequality is from the third condition. We then apply the first condition to obtain $|u[T]| \preceq \bar{u}$, and thus $\begin{bmatrix} y[T] \\ u[T] \end{bmatrix} \in \SigSp{I}$. Using mathematical induction, we conclude that $\begin{bmatrix} y[t] \\ u[t] \end{bmatrix} \in \SigSp{I}$ for all $t$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{lemma:Hinf}]
This is a direct application of the small gain theorem \cite{zhou1996robust}. We have
\begin{subequations}
\begin{align}
\| \tf y \|_{\ell_2} &= \| \tf{\Phi_{yw}} \tf w + \tf{\Phi_{yu}} \tf u \|_{\ell_2} \label{eq:small1}\\
&\leq \| \tf{\Phi_{yw}} \tf w \|_{\ell_2} + \|\tf{\Phi_{yu}} \tf u \|_{\ell_2} \label{eq:small2} \\
&\leq \| \tf{\Phi_{yw}}\|_{\mathcal{H}_\infty} \|\tf w \|_{\ell_2} + \|\tf{\Phi_{yu}} \|_{\mathcal{H}_\infty} \|\tf u \|_{\ell_2} \label{eq:small3} \\
& \leq \| \tf{\Phi_{yw}}\|_{\mathcal{H}_\infty} \|\tf w \|_{\ell_2} + \|\tf{\Phi_{yu}} \|_{\mathcal{H}_\infty} \gamma \|\tf y \|_{\ell_2}. \label{eq:small4}
\end{align}
\end{subequations}
where \eqref{eq:small2} comes from the subadditivity property of a norm and \eqref{eq:small3} from the fact that $\mathcal{H}_\infty$ norm is equivalent to the $\ell_2$ to $\ell_2$ induced norm. By assumption, we have $\|\tf{\Phi_{yu}}\|_{\mathcal{H}_\infty} \gamma < 1$. Therefore, we have
\begin{equation}
\| \tf y \|_{\ell_2} \leq (1 - \gamma \|\tf{\Phi_{yu}}\|_{\mathcal{H}_\infty})^{-1} \| \tf{\Phi_{yw}}\|_{\mathcal{H}_\infty} \|\tf w \|_{\ell_2},
\end{equation}
which means that the $\mathcal{L}_2$ gain from input $\tf w$ to output $\tf y$ is bounded. This implies input-output stability of the closed loop system.
\end{proof}

Without losing generality, we assume $\| \Delta \|_{\mathcal{L}_1} \leq 1$. With this assumption, we always have $\| \ttf{\delta} \|_{\ell_\infty} \leq \| \ttf{\alpha} \|_{\ell_\infty}$. To show stability, we first require $\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1} < 1$ so that the loop between the plant and the uncertainty $\tf{\Delta}$ is stable. We then have
\begin{subequations}
\begin{align}
\| \ttf{\delta} \|_{\ell_\infty} & \leq \| \ttf{\alpha} \|_{\ell_\infty} \nonumber\\
&= \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w + \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \ttf{\delta} \|_{\ell_\infty} \nonumber\\
&\leq \| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1} \| \ttf{\delta} \|_{\ell_\infty} + \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w \|_{\ell_\infty}.
\end{align}
\end{subequations}
From the assumption $\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1} < 1$, we have
\begin{equation}
\| \ttf{\delta} \|_{\ell_\infty} \leq (1-\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1})^{-1} \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w \|_{\ell_\infty}    
\end{equation}
Then, we have
\begin{subequations}
\begin{align}
\| \tf y \|_{\ell_\infty} & \leq \| \tf{\Phi_{y \ttf{\delta}}}\|_{\mathcal{L}_1} \|\ttf{\delta}\|_{\ell_\infty} + \| \tf{\Phi_{yu}} \tf u + \tf{\Phi_{yw}} \tf w\|_{\ell_\infty} \nonumber\\
&\leq \| \tf{\Phi_{y \ttf{\delta}}}\|_{\mathcal{L}_1} (1-\| \tf{\Phi_{\ttf{\alpha} \ttf{\delta}}} \|_{\mathcal{L}_1})^{-1} \| \tf{\Phi_{\ttf{\alpha} u}} \tf u + \tf{\Phi_{\ttf{\alpha} w}} \tf w \|_{\ell_\infty} + \| \tf{\Phi_{yu}} \tf u + \tf{\Phi_{yw}} \tf w\|_{\ell_\infty}
\end{align}
\end{subequations}
